Mechanical TA 2: A System for Peer Grading with TA Support

Mechanical TA 2 (MTA2) is an open source web-based peer grading application that leverages trusted TA graders to incentivize high-quality peer review. A previous, prototype implementation of MTA proved the value of the concept, but was neither suitable for use at scale nor easily extensible; MTA2 is a complete reimplementation of the system that overcomes these hurdles. MTA2 serves two, interconnected purposes: facilitating practical peer grading and serving as a testbed for experimentation with different peer grading mechanisms. The system is characterized by a modular design that makes customization easy; support for dividing students into different pools based on their peer-grading prowess; mechanisms for automated calibration and spot checking; and the ability for students to appeal grades and to give feedback about individual reviews.

==> MTA2 paper- Arxiv/abstract.tex <==
%This
% paper
%article
%describes \emph{Mechanical TA 2} (MTA2), a web-based peer grading application.
% The key difference from other peer-grading systems is that, instead of trying to remove the role of teaching assistants, it uses their limited availability to create a more reliable system.
%The existing peer grading applications have tried to remove the role of teaching assistants. However, MTA tries to make use of their limited availability in order to create a more reliable system.
%An initial implementation of MTA proved
% the value of the concept,
%the effectiveness of the underlying idea
%but was built in a way that limited its
% effectiveness
%use cases
%both for
% use
%being deployed
%at scale and for easy extensibility. MTA2 is designed and created
% by having the following two goals:
%with the following goals in mind:
%to provide a practical peer-grading system for general use and to serve as a testbed for experimentation with different peer grading mechanisms. Key features in MTA2 are its modular design which makes it easy to customize, the support for having multiple pools of students, automated calibration and spot checking mechanisms, and the ability for students to appeal an unfair grade as well as flagging individual inappropriate reviews. 

\emph{Mechanical TA 2} (MTA2) is an open source web-based peer grading application that leverages trusted TA graders to incentivize high-quality peer review. A previous, prototype implementation of MTA proved the value of the concept, but was neither suitable for use at scale nor easily extensible; MTA2 is a complete reimplementation of the system that overcomes these hurdles. MTA2 serves two, interconnected purposes: facilitating practical peer grading and serving as a testbed for experimentation with different peer grading mechanisms. The system is characterized by a modular design that makes customization easy; support for dividing students into different pools based on their peer-grading prowess; mechanisms for automated calibration and spot checking; and the ability for students to appeal grades and to give feedback about individual reviews. 

==> MTA2 paper- Arxiv/conclusion.tex <==
Mechanical TA 2 (MTA2) is an open source, web-based peer grading application that leverages trusted TA graders to overcome three main drawbacks in traditional peer grading: incentives, standardization, and leverage. The system is designed both to facilitate practical peer grading and to support research and experimentation about the design of peer grading mechanisms. MTA2 is characerized by a modular design that makes customization easy; support for dividing students into multiple pools based on their peer-grading ability; mechanisms for automated calibration and spot checking; and the ability for students to appeal grades and to flag inappropriate reviews. 

%MTA2 is a complete reimplementation of a previous prototype system (MTA1). 

In future work, we plan to experiment with different peer grading mechanisms using MTA2. We are sure that these experiments will lead us to continued work on the system's user interface and features. 

==> MTA2 paper- Arxiv/evaluation.tex <==


To date, MTA2 has been deployed in three computer science courses, focused respectively on 
%'s new design and features such as supporting different assignment formats have allowed us to use the system in several different computer science courses: 
algorithms, programming, and computers and society. We have not run a formal user study to evaluate MTA2's new design, but have informally received considerable positive feedback from students and instructors who used the system. In the case of the computers and society course, we have access to some data about the deployment that is worth summarizing here. 

The computers and society course had 117 students, 11 assignments, 1203 student submissions, 77 calibration essays, 460 TA reviews, and 75 appeals. Figure~\ref{fig:ind_percentage} shows the percentage of students assigned to the independent pool for each assignment~\footnote{For this course, the rule for getting students to the independent pool was slightly more strict than the one described in Section 3.3.}. Observe that by the first assignment, about 40 percent were promoted based on calibration reviews; by the second assignment about 80 percent were promoted, based both on additional calibration and their peer reviews of assignment 1. After this point, the percentage of students in the independent pool fluctuated, due to some students being demoted to the supervised pool. Such demotions were triggered by spot checks, appeals, and reports of individual bad reviews. Overall, these percentages remained around 80 percent, showing that the system succeeded in motivating the vast majority of students to perform high quality peer reviews.
\begin{figure}[t]
	\centering
	\includegraphics[scale=0.46 ]{images/ind_perc.png}
	\caption{The percentage of independent students as a function of assignment number}
	\label{fig:ind_percentage}
\end{figure}



We conducted an end-of-year survey to help us to improve the next course offering. While it was not designed as a research instrument, two categories of responses are useful for investigating the effectiveness of MTA2's design. 
%In the first offering of the course, there were 1248 submissions, 448 TA reviews, and 118 appeals. 
First, two questions asked students about how they learned to improve the quality of their peer reviews. Students reported that TA feedback and calibration reviews were  almost equally effective (see Figure~\ref{fig:ta_vs_cal}); however, note that the distribution of support for TA feedback stochastically dominates that of calibration reviews (i.e., students preferred to receive TA feedback). %This could be due to the fact that TA feedback directly address students' individual reviews and helps them understand their mistakes better. 

\begin{figure}[t]
	\centering
	\includegraphics[scale=0.46 ]{images/ta_vs_cal.png}
	\caption{Students' answer to the two questions about how they learned to improve the quality of their peer reviews. The results show that TA feedback and calibration reviews were almost equally useful}
	\label{fig:ta_vs_cal}
\end{figure}

Second, we asked students how user friendly they found the MTA2 interface. Overall, 69\% scored the user interface either 4 or 5 out of 5 (see Figure~\ref{fig:user_interface}). We contrast this with the system's initial implementation (MTA1); while we are aware of no comparable survey data, that system received many oral and written complaints about its user interface, which indeed served as one of the motivations for our system redesign.

\begin{figure}[t]
	\centering
	\includegraphics[scale=0.46 ]{images/user_interface.png}
	\caption{MTA2 user interface ranking}
	\label{fig:user_interface}
\end{figure}


%in both years what percentage of the feedback that they got from peer reviews they felt indicated that their peer reviewer invested an adequate degree of effort reviewing their essay. Figure~??? shows the result of this survey. 

%\subsection{Standardization}

%\subsection{Leverage}


%\subsection{User interface}

==> MTA2 paper- Arxiv/features.tex <==


%\subsection{Modular design}
 %MTA has a modular design, which allows instructors to choose their desired features in their course. For example, an instructor can choose whether to have independent/supervised pools (see section~\ref{subsec:pools}) or calibration (see section~\ref{subsec:calibration}) in the system or no. Moreover, the modular design makes it easy for users to edit each feature to meet their specific requirements. For example, if an instructor wants to change the way grading load is distributed among peers or modify the algorithm by which spot checks are assigned, they can easily do that by editing their corresponding functions in the code base, without having to worry about the functionality of other parts of the system. 
%\begin{itemize}
%    \item What do we mean by modular design?
%    \item why is it helpful?
%    \item How it is done in MTA2?
%\end{itemize}

In this section, we describe MTA2's key features. We explain how these deliver the properties discussed in the introduction (incentives, standardization, and leverage) and help MTA2 to be a high-performance, reliable, and extensible peer grading application.  %Note that among these features the early versions of supervised and independent pools, spot-checking, and calibrations already existed in MTA1 and are only revised in MTA2. However, the modular design, flagging individual reviews and easy integration with CAS and SAML2 features are newly introduced by MTA2. 


%\subsection{Modular design}
% Many of MTA1's design choices are hard coded, making the system difficult to change. In contrast, MTA2 offers a modular and easy-to-manipulate design, with the goal of realizing two key benefits.  First, we wanted to make it easier for instructors to choose the features they need for their own course workflows. Second, we wanted to facilitate the system's use for research into peer grading incentive mechanism design.

MTA2 makes it possible for instructors to toggle any of the following features: supervised and independent pools, calibration, spot-checking, giving feedback about individual reviews, and integration with SAML2; we will go on to describe each of these features in turn. For users requiring finer grained customization, the MTA2 codebase is written in Python, which makes modifying its behavior simple. The source code is divided into eight directories based on function: assignment, review, evaluation, calibration, grade, account, course, and homepage. The contents of each of these directories is further decomposed into three parts: \textit{templates and views}, which control the UI; \textit{base}, which contains the logic; and \textit{models}, which contain the definitions of data types. 
Hence a newcomer attempting to modify a specific behavior can quickly identify the part of source code that requires modification. For example, by default, MTA2 calculates final grades by taking the median of the grades given to each submission. However, an instructor might prefer a more complicated grade aggregation algorithm, such as Olympian Average. To modify the grade calculation logic one needs only to modify the \texttt{base.py} script inside the \texttt{peer\_grade} directory.

\subsection{Incentives}
MTA2 uses four main features to provide students with sufficient incentives for accurate grading: spot checks, appealing, giving feedback about individual reviews, and using the consensus grade .
%\begin{itemize}
%    \item What is spot-checking?
%    \item Why is it needed?
%    \item how it is done in MTA2?
    
\subsubsection{Spot checking}
In MTA2, a spot check has two parts. The first is a \emph{TA review} of the assignment: the chosen assignment is graded by a TA, using the same grading rubric used by students. Second is \emph{TA evaluation} of the peer graders: the TA uses a separate rubric to evaluate the reviews submitted by students who graded the spot checked assignment, giving a grade on a 10-point scale. %This mechanism as well as appealing and flagging of individual reviews that we will introduce in \autoref{subsec:appeals} and \autoref{subsec:flag_reviews} not only help with incentivizing students to grade their peers more fairly, but also keep the quality of the grades high.
By default, the system lets the instructor choose the number of assignments that need to get spot checked and assigns TAs to students uniformly at random. However, this logic can be revised easily, for example targeting high grades. 
%\klb{Why wouldn't we do this by default?}
%Remember that the modular design of MTA2 allows instructors to easily customize the way that the spot-checks are assigned.
%\end{itemize}
Furthermore, TAs are free to browse through assignments and conduct additional spot checks, based e.g. on reviewer identity, degree of agreement between reviewers, or peer grade assigned.
\subsubsection{Appealing}

Students can appeal when they disagree with a grade assigned by peer reviewers. If the appeal provides a convincing argument, instructors or TAs regrade the assignment and also evaluate every peer review that the assignment has received.

\subsubsection{Giving feedback about individual reviews}
MTA2 also allows students to provide feedback about individual reviews. The procedure is similar to appealing, but it is supported via a separate mechanism for two reasons. First, we found it useful to allow students to identify rude, unfair, or low quality reviews even when these reviews do not affect the student's overall grade. If a student believes that a review is inappropriate, they can flag the review and provide their reasoning. The report is then assigned to a TA as in an appeal. If the TA confirms that the report is inappropriate it no longer affects the assignment's grade. The reviewer is also notified and the TA may take additional action outside the MTA2 system. Second, we wanted to allow students to give positive feedback about particularly good reviews, to help reward students for making exceptional efforts.
%In our early experiments with MTA2, we figured that it is important to recognize the effort of those students who put much more work than others in reviewing their peers. This feature allows the instructors for find such students and take further actions to reward them for their effort.

\subsubsection{Using the consensus grade}

When an assignment is not spot checked, instructors can choose to reward graders by measuring how close their grades are to the consensus grade. We note, however, that recent work has shown that the inclusion of such a mechanism \emph{increases} the amount of spot checking required to provide strong incentives to graders~\citep{gao2016incentivizing}; thus, it is not enabled in MTA2 by default.
%\subsubsection{Evaluation (grading the reviews)}
%\begin{itemize}
%    \item Why do we need evaluations?
    

    
%    Our solution to this problem is to use randomized TA checks, also known as spot-checking.
%    \item how do they happen?
%    \item when do they happen?
%\end{itemize}

\subsection{Standardization} \label{subsec:calibration}
There are two main ways that MTA2 facilitates standardization.

\subsubsection{Calibration submissions}

Calibration submissions have known ``ground truth'' grades; for example, they might be carefully graded submissions from previous offerings of a course. They are graded using the same rubric as student submissions and can either be presented separately to students in the UI (to support a workflow like requiring a calibration review before peer reviews) or mixed together with student submissions (to drive TA spot checks by detecting students who grade poorly).
MTA2 auto-grades calibration reviews by starting with 10 points and then, for each rubric question, subtracting the square of the difference between the student grade and the ground truth grade. For example, if there are two rubric questions and a review is off by one for two of the questions, the score is $10-1^2-1^2=8$. If the review is off by two for only one question, the score is $10-2^2=6$. This is motivated by the idea that a student who understands how to grade well might make small errors, while bigger errors reflect more fundamental misunderstandings. Of course, this formula can be easily changed.
%\begin{itemize}
%    \item What is calibration?
%    \item why it is needed?
%    \item what are the challenges?
%\end{itemize}

\subsubsection{TA and instructor feedback}

TAs and instructors have the opportunity to give student graders feedback about their reviews whenever a submission is spot checked or appealed. This personalized feedback provides another avenue for students to standardize their understanding of the grading rubric. %, and when a review is flagged or is requested for evaluation by a TA.

\subsection{Leverage: Supervised/independent pools} \label{subsec:pools}

MTA is able to maintain different \emph{pools} of students, where students are only assigned peer reviews for others in the same pool.
The first, ``supervised'' pool guarantees that every submission and review submitted by students will also be graded by a TA, with only the TA grade counting for evaluation. The purpose of this pool is to ensure that students do not assign binding peer grades until they have shown themselves to be fair and consistent graders. At the beginning of the course, all students are assigned to the supervised pool. They graduate to the second, ``independent'' pool by demonstrating consistent performance either in calibration reviewing or in real peer review in the supervised pool. (Recall that both calibration reviews and peer-grading reviews are assessed on 10-point scales. By default, MTA promotes a student to the independent pool once they obtain at least 35 points over their five most recent peer-grading or calibration reviews.) Students in the independent pool are evaluated for the quality of their grading only if they are spot checked, the submission they have graded is appealed, or their review is flagged as inappropriate. 


%In our early experiment with MTA2, this promotion rule was not as effective as we hoped. Some students could get into the independent pool by giving average grades to every calibration assignment.  We plan to change this rule in the future iterations of using MTA2. 

The use of supervised and independent pools offers a second benefit for calibration: they dramatically reduce TA grading when a new course starts. Performing calibration reviews can help supervised students to become independent more quickly---often, even before submitting the first assignment. Instructors can also require supervised students to perform additional, weekly calibration reviews, both to reduce TA workload and to help weaker students to learn to peer grade effectively. 


%\begin{itemize}
%    \item What are these pools?
%    \item why do we need them?
%    \item how do they work in MTA2?
%\end{itemize}


%\subsection{Dynamic user interface}
%\input{userinterface.tex}

\subsection{Other major features}
MTA2 also has a variety of new features that do not directly address incentives, standardization or leverage. Here we describe a two of the most important.

% \begin{itemize}
%     \item How does this work? \farzad{Do they get to provide reasoning?}
%     \item Why did we need to add it? Appeal refers to the overall grade which might be unchanged even in the presence of a bad review.
% \end{itemize}

%\subsection{Built-in quiz}

%\begin{itemize}
%    \item What is this?
%    \item Why do we need it?
%    \item How does it work?
%\end{itemize}

\subsubsection{Different assignment types}
In MTA2, an assignment can be created by specifying the assignment's name, type, problem statement, release date, and deadline.%~(see figure~\ref{fig:assgn-creation}). 
Instructors and TAs can also set a late unit period for an assignment, which is the number of days the students' submissions are allowed to be late. MTA2 keeps track of the total number of late days each student has accumulated across the whole course. Once this number reaches the limit set by the instructor at the beginning of the course, the system stops accepting late submissions. In addition to the late unit period, an assignment can also have a grace period, which is a short amount of time after the deadline during which the submission will not be considered late. %This is meant to excuse last-minute emergencies such as connection shortages or other technical issues. 
MTA2 supports three types of assignments.

\minisec{Text} Students submit answers by typing text directly into a text box. Instructors can set a limit for the number of characters or words that can be submitted.

\minisec{Upload} Assignments can also be configured to solicit the upload of PDF, text, or code files. Uploaded files are rendered in the browser directly. When code is submitted, MTA2 highlights syntax automatically. Instructors can also upload a group of student submissions as a zip file, with each student's submission named as their MTA username. This feature lets instructors use the grading features of MTA2 for exams and assignments that happen outside the MTA2 framework.

\minisec{Quiz} Assignments can be multiple-choice quizzes, which can be graded automatically. The system can be configured to show students only final grades (not correct answers) after submission. Instructors can make a quiz a requirement for doing other types of assignments, which is helpful for making sure that students satisfied a prerequisite (e.g., did a reading) before submitting. The instructor can limit the number of times a quiz can be submitted.

%\begin{figure*}[t]
 %   \centering
 %   \includegraphics[scale=0.23]{images/create_assignment.png}
 %   \caption{Creating an assignment.}
 %   \label{fig:assgn-creation}
%\end{figure*}


\subsubsection{Easy integration with SAML2}
%\farzad{We don't have the CAS integration right now. It should be merged, but we don't have access to the new repo yet.}
Security Assertion Markup Language 2.0 (SAML 2.0) defines standard protocols for the exchange of authentication and authorization between domains. It can be used to provide cross-domain single sign on. In many universities and different organizations, users have a universal account that can be used to log into different applications provided by that organization. MTA2 can be integrated into such systems that use the SAML2 standards and can therefore delegate the administration of user accounts to the central organization.
%
%This way the students can simply use their centralized credentials instead of creating a new username and password specifically for MTA2. This also alleviates some of the privacy concerns of the organization or the users about the safety of their data as the user information stored within the MTA2 application itself is minimized.
%
Internally, we use the \texttt{django-saml2-pro-auth} package which is a wrapper for the \texttt{python-saml} package.
%the exchange of public keys and pointing the system to the correct end-points on the centralized login system.
%The settings are combined in a single file and SAML2 login can be enabled or disabled easily.



==> MTA2 paper- Arxiv/figure.tex <==
    
%    \begin{figure*}[ht]
%    \centering
%    \includegraphics[scale=0.23]{images/review_example.png}
%    \caption{A sample review.}
%    \label{fig:review_example}
%\end{figure*}



\begin{figure*}
\centering
\begin{subfigure}[t]{.485\textwidth}
    \vskip 0pt  % top-align
    \centering
    \includegraphics[width=1\linewidth]{images/instructor_dashboard_3.png}
    % \caption{Instructor's view.} 
    % \label{fig:instuctor_dashboard}
\end{subfigure}
\begin{subfigure}[t]{.51\textwidth}
    \vskip 0pt  % top-align
    \centering
    \includegraphics[width=1\linewidth]{images/student_dashboard_3.png}
    % \caption{Students' view.}
    % \label{fig:student_dashboard}
\end{subfigure}
\caption{The dashboard tab for the instructor (on the left) and the students (on the right).}
\label{fig:dashboard_tab}
\end{figure*}

==> MTA2 paper- Arxiv/intro.tex <==


%    \item What Peer grading is, how it helps, what the challenges are.


\newcommand{\minisec}[1]{\vspace{.4em}\noindent\textbf{#1.~}}

Peer grading can improve students' learning of course material by encouraging critical thinking about the work of their classmates and can also help with the delivery of large classes by reducing grading work for teaching assistants (TAs) and instructors~\citep{sadler2006impact}. 
A wide variety of different peer grading systems already exist~\citep{de2014crowdgrader,Calibratedpeerreview,Peergrade,gehringer2001electronic,pare2008peering}; we survey them in Section~\ref{sec:relatedwork}. All of these systems either work without relying on TAs at all or use TAs only at a very basic level (e.g., resolving student appeals). This is appropriate for courses with extremely inadequate numbers of TAs, such as free massive, open, online courses (MOOCs)~\citep{kulkarni2013peer}. But when more TAs are available (e.g., in many university classes with a few hundred students), they can help to overcome three key drawbacks with current peer grading systems, which we dub \textit{incentives}, \textit{standardization}, and \textit{leverage}.

\minisec{Incentives} Peer grading systems only work when students take their grading tasks seriously. While some students behave altruistically or recognize that peer grading helps their own learning, others are motivated by more immediate incentives, e.g., save time by not putting in the effort to grade others.
%Achieving these properties is not easy in large classes, and would require careful design and proper incentive mechanisms for students to behave as intended. 
Many peer grading systems allow students to appeal when they disagree with a peer review \citep{de2014crowdgrader,Peergrade}; this has the effect of discouraging reviewers from giving low grades. Some systems further reward students for choosing grades that are similar to those assigned by other peers to the same submissions~\citep{de2014crowdgrader,hamer2005method}. Unfortunately, neither of these mechanisms discourages students from giving very high grades to every single submission~\citep{de2016incentives,gao2016incentivizing}, offering students a low-effort alternative to grading sincerely. Experimental evidence shows that human subjects do respond to these incentives \citep{gao2014trick}; we have also observed such behavior in our own classroom teaching.
%

TAs can overcome this problem by ``spot checking'' a randomly chosen fraction of submissions  \citep{jurca2005enforcing,wright2015mechanical,gao2016incentivizing,zarkoob2019report}. When a submission is spot checked, a TA grades the submission carefully, evaluates the reviews given to that submission, and rewards or punishes the graders (based on the quality of the feedback they offered, the distance between their assigned grades and the TA grades, or other factors). When spot checking is performed to a sufficient degree, students stand to lose more than they stand to gain from dishonest grading, and hence they have strong incentives to grade sincerely \citep{de2016incentives,gao2016incentivizing}. 

%\farzad{We can mention that even in the absence of collusion, grading students by closeness of their grade to their peers leads to a "race to mediocrity" (Keynesian Beauty contest).}
%\hedayat{Sure, go ahead and do so. Then, we can decide if we want to keep it}

\minisec{Standardization} Peer grading systems should teach students to grade consistently and accurately. Otherwise, different students are likely to assign different grades to the same work~\citep{Calibratedpeerreview,wright2015mechanical,wang2019your,kulkarni2013peer}. There are two key ways that TAs can help in this task. The first is by preparing so-called \emph{calibration submissions}, such as submissions from previous years, which can then be assigned to all students in the class \citep{Calibratedpeerreview}. Immediately after a student grades a calibration submission, they can be shown the TA grade and given its rationale; such instantaneous feedback has been shown to aid learning \citep{kulik1988timing}. The second is to let TAs give personalized feedback to students on their grading performance. Calibration can work with very limited TA resources, but of course it is also valuable to have TAs provide direct feedback on actual peer grading (triggered, e.g., by a student appeal, a random spot check, or some other signal such as a pattern of suspiciously similar grades). %\farzad{I never understood how this happens. TAs are busy, I imagine they would look at an assignment only if there was an appeal/flag.} 
%Although providing such feedback inevitably takes longer in this approach, TAs can look at a review given by a student to a submission and give direct feedback on how the submitted review could be improved.   

\minisec{Leverage} Peer grading systems must find a way to rely on students who are able to grade their peers reliably---and hence need a relatively low level of supervision---without being derailed by others who are less skilled or more erratic peer graders. In order for a peer grading system to scale, it must trust students who have demonstrated competence. However, students who struggle to grade accurately can lower the average quality of peer grades and undermine student acceptance of the system. TAs can be useful both for identifying such students and for helping to teach them how to grade more effectively.

% this describes the solution, not the property.
%Even after performing calibration reviews and getting feedback from TAs, not every student is going to qualify for grading their peers accurately. At the same time, an efficient peer grading system should take advantage of those students whose grading performances reach a certain level of proficiency; Once a few of qualified students grade a submission, it is very likely that there is no more need for a TA to look at the submission. This scenario can be taken into consideration by allowing instructors to divide students into two pools: independent and supervised, where students in each pool are only assigned to grade those in the same pool~\citep{wright2015mechanical}. Every submission and review submitted by students in the supervised pool will also be graded by a TA. At this stage, students are learning to be fair and consistent graders. At the beginning of the course, all students are in a supervised pool. However, supervised students have the ability to move to the independent pool by showing consistent performance either by accurately grading a set of calibration submissions or by being evaluated by TAs multiple times. After a student gets into the independent pool, their grading will be evaluated by TAs only if they are spot checked, the submission they have graded is appealed, or their review is flagged as inappropriate. 

\emph{Mechanical TA} (MTA) is a system that facilitates peer grading with TA support; it provides all three of the properties just discussed (incentives, standardization, and leverage). We survey key properties of the system in Section 3. A prototype implementation of MTA (MTA1) was used in a computer science course called ``Computers and Society'' for several years. A study published at SIG-CSE \citep{wright2015mechanical} demonstrated the system's usefulness: specifically, MTA1 significantly reduced the need for TA labor in a large class and its use of spot checking, calibration, and division of students into multiple pools helped students to grade more accurately and to learn the course material. However, MTA1 was highly specialized to the Computers and Society course and many of its design choices were hard coded, making the system difficult to change, which limited its usefulness in other settings. 
%MTA2 is created based upon MTA1 to resolve its limitations and also to be a reliable and flexible peer grading application which can be used in various different settings. %It is easy to modify for courses with different requirements and supports new features that are helpful to have in a practical peer grading system. 
%In many scenarios such as university classes, the instructor indeed has access to a limited TA resource. 

%Similar to MTA1, TAs play a limited but important role in obtaining reliable grades in MTA2. 





%To obtain accurate grading and avoid students' collusion, MTA2 takes advantage of the limited availability of TAs in three main ways: 



%Spot checking also results in a fraction of final grades be TA grades in the system, which are expected to be more accurate than peer grades. Therefore, overall, the system would end up having more accurate grades.  

MTA2 is a complete reimplementation of MTA that improves performance, reliability, and extensibility and also introduces various new features. The design of MTA2 has modularity at its core, allowing 
%One of the key new features of MTA2 is its modular design. As mentioned, MTA1 used several helpful features such as spot-checking to build a more reliable peer grading system. Such features are helpful to have in a peer grading system, however, not every instructor can afford to have them in their course. The modularity of MTA2 lets 
instructors to choose the features they want based on the workload of their courses and making it easy to change system logic like the rules according to which students move between pools. As already indicated, the design of peer grading mechanisms is an active area of academic research; MTA2's modular design also makes it a good environment for evaluating such mechanisms (e.g., different spot checking or grade aggregation mechanisms). 
%There are many important unanswered questions about building a practical peer grading system. For example, as mentioned, MTA's way of incentivizing accurate grading among students is to spot check them. However, finding the most efficient spot checking mechanism is still an open problem in many scenarios~\citep{zarkoob2019report}. MTA2 has not only made it easier for instructors to choose the features they want, but also to modify and test them in practice. 
To our knowledge, MTA2 is the first peer grading application that offers this level of flexibility. %For example, an instructor can change the way that submissions are distributed among peers for grading or modify the algorithm by which spot checks are assigned, without having to worry about the functionality of other parts of the system.

%MTA2's flexibility along with some additional features help the system to work better in practice and also serve as a testbed for experimenting with different peer grading mechanisms.
%and was done in a way that the logic and the user-interface of the system were mixed together.  
%Although 

Beyond its architectural advantages, MTA2 also offers four key new features that make it applicable in a much wider range of contexts than MTA1. First, MTA2 allows students to submit assignments as ASCII text, PDFs, or answers to multiple choice questions~\footnote{MTA1 only supported plain text.}. 
%Depending on the assignment type, MTA2 allows students to input text, upload a file, or choose one of the multiple choices as their solution. 
When text, PDF, or code files are uploaded, the result is rendered directly in the browser (e.g., for grading) rather than needing to be downloaded. Second, students can flag inappropriate reviews independently of the appeal process. This is important because it is a best practice to aggregate peer grades in a way that reduces sensitivity to outliers \citep{hamer2005method}, e.g. by taking the median of peer grades. While this makes grading fairer, it also means that students may not be motivated to appeal when they receive a single inappropriate review. In our early deployment of MTA2, we found that this change can lead to a considerable increase in student satisfaction. % When a grade is appealed, a TA looks at the reasoning and if necessary and regrades the student's submission. The TA can also evaluate any of the reviews done for this submission. But, flagging individual inappropriate reviews is %\farzad{Can't we just do this computationally? I thought flagging was mostly used for "inappropriate" reviews (rude, etc?).}
Third, MTA2 allows instructors to upload groups of student submissions as a single zip file. This allows the ingestion of exams and quizzes conducted outside of MTA, allowing them to be peer graded as well. %All an instructor has to do to make this happen is to create an assignment in MTA2 and upload PDFs of scanned student submissions \farzad{too much detail, I suggest cutting off "named by students' usernames "} as a single zip file. 
Finally, MTA2 offers advanced SAML2 integration, allowing users to log in using  organizational accounts (e.g., university-wide login systems), increasing ease of use, security, and regulatory compliance.
     
   
The rest of this paper is organized as follows. Section~\ref{sec:relatedwork} describes existing peer grading systems and explains how they differ from MTA2. Section~\ref{sec:features} introduces the main features of MTA2 and Section~\ref{sec:userinterface} describes the main components of the system's user interface. %In Section~\ref{sec:backend}, we briefly go over the code base of MTA2, its general structure, and explain the way some of its core algorithms can be modified.  
Section~\ref{sec:evaluation} describes deployment of MTA2 and Section~\ref{sec:conclusion} concludes and discusses future directions. 



==> MTA2 paper- Arxiv/relatedwork.tex <==
%Many implementations of peer grading systems already exist, each of which use different mechanisms to overcome practical issues associated with peer grading. 
%Now that we have discussed the main drawbacks of peer grading systems, in this section, we go over the most notable implementations of peer grading systems and point out their mechanisms to overcome these drawbacks and their differences with MTA2. 
To our knowledge, Calibrated Peer Review (CPR)~\cite{Calibratedpeerreview}, Crowdgrader~\citep{de2014crowdgrader}, Peer Grader (PG)~\citep{gehringer2001electronic}, PeerScholar~\cite{pare2008peering}, and Peergrade~\citep{Peergrade} are the most commonly used peer grading applications.  Tables~\ref{table:comparison} and~\ref{table:featurecomparison} give an overview of MTA2, MTA1, and each of these applications, comparing them in terms of incentives, standardization, and leverage, and also in terms of several desirable system properties. 
%However, imagine a scenario in which, instead of individuals, large groups of students collude on not putting in the grading effort and giving each other high grades. The appealing mechanism fails to detect such undesirable behavior because students are not going to complain about high grades\footnote{It is also worth mentioning that some researchers have suggested using rewarding mechanisms based on similarity measurement between the grades that students report. Unfortunately, all of those mechanisms are also prone to the collusion of students on reporting high grades.}.
%\klb{Why did the list of desiderata change to these 7 in particular? If you're going to go beyond the 3 in the intro, are there other topics you should also list? (E.g., can students appeal? Can students see their grades? What about the four new features described at the beginning of the introduction?)}

Calibrated Peer Review (CPR)~\cite{Calibratedpeerreview} is designed for reviewing writing assignments. CPR pioneered the use of calibration submissions to help students standardize their grading. The system requires students to perform such calibration before grading each assignment. MTA2 largely follows CPR in its use of calibration, except that it allows students who have demonstrated grading proficiency to stop performing calibration.
% KLB: why so much about MTA here? It's a related work section.
% However, in many scenarios such as essay writing assignments, reviewing can be a time-consuming task. Also, grading criteria does not change much from one assignment to another. Therefore, CPR can put an unnecessary grading load on students for each assignment. In MTA2, once students show consistency in reviewing others at any time during the course, they can keep reviewing their peers, unless a TA disqualifies them by looking at their grading history. Note that in MTA2, a qualified grader can always request to review optional calibration submissions to improve their confidence in grading new assignments. 
CPR uses a consensus grade for each assignment to give students some incentive for grading accurately, though it does not offer a mechanism for discouraging all students from reporting high grades.
%\klb{Should you mark this as partial provision of incentives?}
 
CrowdGrader~\citep{crowdgrader_2013,de2014crowdgrader,crowdgrader_2016} and PeerGrade~\citep{Peergrade} are two commercial peer grading web application and provides many useful features to the instructor~(see Table~\ref{table:featurecomparison}). They have been built to be fast, simple, and scalable to large class sizes. Similar to CPR, CrowdGrader gives students partial incentives via a consensus grade mechanism. PeerGrade aims to incentivize accurate grading by asking reviewers to evaluate each other's reviews. (Note that this does not provide stronger incentives in a game theoretic sense; as before, students can avoid performing the effort of sincere reviewing if they all simply give each other high grades.) %PeerGrade supports different assignment types and allows students to flag individual reviews, but it does not support calibration.
 

%\klb{These descriptions should start with one or two sentences saying what the peer grading system's focus is---what does it try to do well, what's its design philosophy, etc.? As it is, the bulk of these descriptions basically just turn the information in the table into sentence form. We have already read the table...}


PG~\citep{gehringer2001electronic} is another peer grading application designed and used for computer science courses. A student in PG can choose either to submit new work or to review the work of other people. PG enables reviewers to communicate with authors during an initial feedback phase, after which authors can revise their submissions; finally, reviewers assign a grade. PG aims to encourage accurate grading by having authors evaluate reviewers. It records the best student submission, allowing it to be used for educational purposes later.  
  
PeerScholar~\citep{pare2008peering} is another application which focuses on implementing peer grading in large classes. Similar to MTA, it started by supporting writing assignments, but, its later versions included different assignment formats. The early version of PeerScholar asked students to write separate essays demonstrating comprehension of an assigned reading and reacting to it; these essays are then peer graded.

% \citep{de2014crowdgrader,gehringer2001electronic,mulder2007praze,pare2008peering,Peergrade} use a consensus grade to reward a student for being accurate or ask the reviewers, themselves, to evaluate each others reviews. As mentioned, such approaches are prone to collusion between students where they can coordinate on always giving high scores to each other's submissions and reviews. 
 

Several further peer-reviewing systems focus on gathering fast feedback on draft versions of a student assignment \citep{cho2007scaffolded,kulkarni2015peerstudio,politz2014captainteach,mulder2007praze}, rather than using these systems to assign final grades. 
%Although these systems are still based on peer review, they are not directly focusing on grading students' final submissions and their goals are mostly different from MTA2. 
Notably, CaptainTech~\citep{politz2014captainteach} used the idea of spot-checking on seeded solutions in a programming course, but in a much more limited way than MTA. Its designers argue that since their system does not use student reviews to calculate final grades, they only lightly used spot checking to check students' feedback quality. 

We are also aware of two more recent peer grading applications: Kritik~\citep{Kritik} and Peerceptiv~\citep{peerceptiv}. Kritik is an AI based peer grading application that focuses on finding fair, accurate, and high quality grades. Peerceptiv is developed based on~\cite{cho2007scaffolded}'s design with data driven algorithms to assign final grades to students.
%\klb{You don't describe what they did precisely enough. What are spot checks used for and why?}
%In MTA2, much of the focus is to make sure that students provide accurate grades to each other and spot checking plays a prominent role in obtaining that.  

%Finally, there are many other peer assessment services designed for use beyond classroom settings. \citep{MyReview,Conftool,Percisionconference} support the review of conference papers; 
%\klb{There are many more: ConfMaster, EasyChair, HotCRP are probably the three most widely used. Plus there are yet other systems for reviewing journal papers.}
%\klb{Give a name}\citep{merrifield2009telescope} supports review of proposals for using telescope time. 
%These systems are all based on peer assessment. However, they are designed for different applications and their mechanisms are mostly similar to the ones we already discussed for other peer grading system. Therefore, we skip talking about the details of their design.
%\klb{What was written here was really weak. It would be great to give a better summary here, else just don't write anything.}

%\begin{itemize}
%    \item Crowdgrader \cite{crowdgrader_2013} argues that even though a system that uses student grades without supervision can be tricked, in practice this is not a huge problem. They observe that in many cases the students are more inclined to reward originality than the TAs. In fact they argue that TAs have an incentive to avoid controversy which negatively influences their grades. The first version of Crowdgrader \cite{crowdgrader_2013} used a reputation-based algorithm to compute the review grades, however, later on  they switched to using Olympic Averaging, which computes the average of all grades except the minimum and the maximum \cite{crowdgrader_2016}. This method is similar to the median of the grades which is used in MTA2.
    
%    \farzad{We can introduce the term ``Keynesian beauty contest'' in the introduction. Having a specific name makes it easier to discuss issues related to the concept.}
    % \begin{itemize}
    %     \item Keynesian beauty contest
    %     \item students are more inclined to reward originality than TAs. All TAs want is avoid controversy
    %     \item reputation-based crowdsourcing algorithm: their later results go against using student reputation as large errors are more correlated with items (hard to grade) than students
    %     \item they later try out feedback to reviews but observe tit-for-tat
    %     \item olympic averaging
    %     \item little correlation between the time it took to perform the review, or how late in the review period the review was performed 
    % \end{itemize}
    
%    \item Peergrader
    
%    \item CPR uses calibration reviews to evaluate each student's grading abilities. The students get a second try if the first review does not meet the instructor's expectations. The quality of the calibration reviews are then used to weight the students' review grades. An issue here is that the quality of student reviews might differ between the calibration and grading phases. MTA2 adopts the calibration idea with some modifications. Most importantly, the calibration is used to determine which students are in the supervised and independent pools but not for the grade calculation.
    
%    \item Telescope
%    \item 
%\end{itemize}

==> MTA2 paper- Arxiv/table.tex <==
\begin{table*}[h]
\centering
 \begin{tabular}{p{1in}p{0.9in} c c c c c c c c} 
 \toprule
 \textbf{Property} & \textbf{Method} &\textbf{PeerScholar} & \textbf{PG} & \textbf{CPR} & \textbf{CrowdGrader} & \textbf{PeerGrade} & \textbf{MTA1} & \textbf{MTA2} \\  
\midrule
\multirow{3}{*}{\emph{Incentives } via}& TA spot checks & -- & -- & -- & -- & -- & \checkmark & \checkmark \\
& grade consensus & -- & -- & \checkmark & \checkmark & \checkmark & -- & \checkmark\\
& review the reviewer & \checkmark & \checkmark & -- & -- & \checkmark & -- & \checkmark \\
\hline
\multirow{2}{*}{\emph{Standardization} via}  & calibration submissions & --  & -- & \checkmark & -- & -- & \checkmark & \checkmark \\
& instructor/TA feedback & --  & -- & \checkmark & \checkmark & \checkmark & -- & \checkmark \\
\hline
\emph{Leverage} via  &dividing graders into pools & -- & -- & -- & -- & -- & \checkmark & \checkmark \\
 \bottomrule
\end{tabular}
\caption{Comparing peer grading applications: Our key desiderata.}
\label{table:comparison}
\end{table*}



\begin{table*}[h]
\centering
 \begin{tabular}{p{1.9in}  c c c c c c c} 
 \toprule
 \textbf{Feature} &\textbf{PeerScholar} & \textbf{PG} & \textbf{CPR} & \textbf{CrowdGrader} & \textbf{PeerGrade} & \textbf{MTA1} & \textbf{MTA2} \\  
\hline
Instructors can enable and disable features  & \checkmark  & -- & \checkmark & -- & \checkmark & -- & \checkmark \\ 
Instructors can change system logic  & -- & -- & -- & -- & -- & -- & \checkmark \\ 
Support for different assignment types & \checkmark  & \checkmark & -- &\checkmark & \checkmark & -- & \checkmark \\
Students can give feedback about individual reviews  & -- & -- & -- & -- & \checkmark & -- & \checkmark \\
Provide data-driven insights to instructors & -- & -- & -- & -- & \checkmark & -- & -- \\
Students can hand in group assignments  & -- & -- & -- & \checkmark & \checkmark & -- & -- \\
Support for checking submission similarity & -- & -- & -- & \checkmark & -- & -- & -- \\
Students and instructors can discuss submissions & \checkmark & \checkmark & -- & \checkmark & -- & -- & -- \\
Instructors can choose to grade individual submissions & -- & -- & -- & \checkmark & \checkmark & -- & \checkmark \\
Easy integration with SAML2 & -- & -- & -- & -- & -- & -- & \checkmark \\
Students can review themselves (self-assessment) & -- & -- & \checkmark & -- & \checkmark & -- & \checkmark  \\
 \bottomrule
\end{tabular}
\caption{Comparing peer grading applications: Other major features.}
\label{table:featurecomparison}
\end{table*}



==> MTA2 paper- Arxiv/test.tex <==


%    \item What Peer grading is, how it helps, what the challenges are.

%\farzad{Apparently, the use of slash ("/") is not recommended in formal writing.} 


Peer grading can help students learn course material better by thinking critically about the work of their classmates. It can also make class sizes scalable by reducing a large portion of grading work for teaching assistants (TAs) and instructors~\citep{sadler2006impact}. However, there are many issues that can stop a peer grading system from achieving these desirable properties in practice, e.g., it is not clear how to make sure that students take their grading tasks seriously or that they know how to grade fairly. 






Many implementations of peer grading systems already exist~\citep{de2014crowdgrader,Calibratedpeerreview,wright2015mechanical,Peergrade}, which either work under the assumption that there is no access to teaching TAs at all or use TAs at a very basic level (e.g., resolving student appeals). However, for the reasons that will be explained in this paper, none of these systems can satisfy all the properties that a reliable peer grading system should have to be confidently used in practice.


\emph{Mechanical TA 2} (MTA2) is a peer grading application designed and developed to overcome practical issues associated with peer grading by leveraging limited access to teaching assistants (TAs). The first implementation of MTA (MTA1),  which was used in a computer science course called ``Computers and Society'' for several years significantly reduced the need for TA labor in a large class, and helped students grade more accurately and better learn the course material ~\citep{wright2015mechanical}. However, the design of the first version was specific to the course it was being used for and was not easy to revise or change, which made it difficult to try in other settings. MTA2 is created based upon MTA1 to resolve its limitations and also to be a reliable and flexible peer grading application which can be used in various different settings. %It is easy to modify for courses with different requirements and supports new features that are helpful to have in a practical peer grading system. 
%In many scenarios such as university classes, the instructor indeed has access to a limited TA resource. 

%Similar to MTA1, TAs play a limited but important role in obtaining reliable grades in MTA2. 



In many peer grading systems, students can appeal unfair grades so that no reviewer can get away with giving grades that are too low~\citep{de2014crowdgrader,Peergrade}. Furthermore, to better incentivize accurate grading, some systems reward their students based on a similarity measurement between grades given by them and by those given by their peers to same submissions~\citep{de2014crowdgrader,hamer2005method}. Unfortunately, collusion between students can trick both of these mechanisms: students can give unfair, but close to full mark grades to every single submission~\citep{de2016incentives,gao2016incentivizing}. This, in turn, dis-incentivizes students from spending time on their grading duties. Experimental studies have shown that this indeed happens in practice~\citep{gao2014trick}. 
\farzad{We can mention that even in the absence of collusion, grading students by closeness of their grade to their peers leads to a "race to mediocrity" (Keynesian Beauty contest).}
\hedayat{Sure, go ahead and do so. Then, we can decide if we want to keep it} MTA2 uses the idea of \emph{spot checking} to detect and avoid defective grading behavior such as collusion. Spot checking is the process of randomly choosing a fraction of submissions and having them graded by TAs. Once a submission is spot checked, a TA grades the submission carefully, evaluates the reviews given to that submission, and rewards or punishes the students based on how close their grades are to the TA assigned grade. If the system spot checks enough submissions, bad grading behaviors such as collusion are likely to be caught, therefore, instead of cheating, students would prefer to focus on their grading duties~\citep{de2016incentives,gao2016incentivizing}. 

%To obtain accurate grading and avoid students' collusion, MTA2 takes advantage of the limited availability of TAs in three main ways: 

A reliable peer grading system should also educate students on how to grade consistently and accurately. Without such an education, it is very likely that because of having different expectations, students would assign different grades to the same work~\citep{wright2015mechanical,wang2019your,Calibratedpeerreview}. MTA2 resolves this issue by two different TA-based approaches. The first approach is to ask students to review \emph{calibration} submissions, which are TA graded submissions from previous years. Once a student finishes grading a calibration submission, they immediately see the TA grade and how different they are from it and can calibrate their grading, accordingly. Such immediate feedback is an efficient way to improve one's performance~\citep{kulik1988timing}. The second approach is to let TAs evaluate reviews given by students to their peers at any time, if necessary (e.g., during an appeal or spot check process). %\farzad{I never understood how this happens. TAs are busy, I imagine they would look at an assignment only if there was an appeal/flag.} 
Although providing such feedback inevitably takes longer in this approach, TAs can look at a review given by a student to a submission and give direct feedback on how the submitted review could be improved.   

Even after performing calibration reviews and getting feedback from TAs, not every student is going to qualify for grading their peers accurately. At the same time, an efficient peer grading system should take advantage of those students whose grading performances reach a certain level of proficiency; Once a few of qualified students grade a submission, it is very likely that there is no more need for a TA to look at the submission. MTA2 takes this scenario into consideration by allowing instructors to divide students into two pools: independent and supervised, where students in each pool are only assigned to grade those in the same pool. Every submission and review submitted by students in the supervised pool will also be graded by a TA. At this stage, students are learning to be fair and consistent graders. At the beginning of the course, all students are in a supervised pool. However, supervised students have the ability to move to the independent pool by showing consistent performance either by accurately grading a set of calibration submissions or by being evaluated by TAs multiple times. After a student gets into the independent pool, their grading will be evaluated by TAs only if they are spot checked, the submission they have graded is appealed, or their review is flagged as inappropriate. 

%Spot checking also results in a fraction of final grades be TA grades in the system, which are expected to be more accurate than peer grades. Therefore, overall, the system would end up having more accurate grades.  

MTA2 improves MTA1's performance and usability by introducing new features. One of the key new features of MTA2 is its modular design. As mentioned, MTA1 used several helpful features such as spot-checking to build a more reliable peer grading system. Such features are helpful to have in a peer grading system, however, not every instructor can afford to have them in their course. The modularity of MTA2 lets instructors choose the features they want based on the workload of their courses. Another important usage for MTA2's modular design is that it makes MTA2 a good environment for testing different peer grading mechanisms. There are many important unanswered questions about building a practical peer grading system. For example, as mentioned, MTA's way of incentivizing accurate grading among students is to spot check them. However, finding the most efficient spot checking mechanism is still an open problem in many scenarios~\citep{zarkoob2019report}. MTA2 has not only made it easier for instructors to choose the features they want, but also to modify and test them in practice. To our knowledge, MTA2 is the first peer grading aplpication with such flexibility. %For example, an instructor can change the way that submissions are distributed among peers for grading or modify the algorithm by which spot checks are assigned, without having to worry about the functionality of other parts of the system.
 
 
In peer grading, grade aggregation methods can be such that having only one unfair grade would not affect students' final grade by much~\citep{hamer2005method}, e.g. by taking the median of reported grades from multiple students. This means that students are not motivated to appeal when they have only one unfair review. However, this should not mean that individual inappropriate reviews would remain hidden from the system. In our early experiments with MTA2, we observed that indeed this scenario happens frequently in practice. Therefore, we added a feature which lets students flag individual inappropriate reviews. % When a grade is appealed, a TA looks at the reasoning and if necessary and regrades the student's submission. The TA can also evaluate any of the reviews done for this submission. But, flagging individual inappropriate reviews is
This gives an opportunity for students to let the system know about inappropriate reviews without going through the whole appealing process. %\farzad{Can't we just do this computationally? I thought flagging was mostly used for "inappropriate" reviews (rude, etc?).}

 

%MTA2's flexibility along with some additional features help the system to work better in practice and also serve as a testbed for experimenting with different peer grading mechanisms.
%and was done in a way that the logic and the user-interface of the system were mixed together.  
%Although 

 
In addition to the modular design and the ability to flag individual reviews, MTA2 supports several other new features that extend its usability in various courses. First, while in MTA1 students could only input their solutions in a text-box, MTA2 supports various assignment formats, i.e., text, PDF, and quiz (multiple choice questions). Depending on the assignment type, MTA2 allows students to input text, upload a file, or choose one of the multiple choices as their solution. In the case of uploading text, PDF, or code files, uploaded files are rendered and shown directly in the browser without needing to be downloaded. Second, MTA2 allows instructors to upload a group of students submissions as a single zip file. This feature would be helpful for exams and quizzes outside the MTA2 framework, allowing them to be peer-graded as well. %All an instructor has to do to make this happen is to create an assignment in MTA2 and upload PDFs of scanned student submissions \farzad{too much detail, I suggest cutting off "named by students' usernames "} as a single zip file. 
Finally, MTA2 has a more advanced CAS and SAML2 integration, which allows users to login using their organizational accounts (e.g., university-wide login systems), without the need for creation of separate username and passwords.
 
     
   
The remainder of this paper is as follows. First, we go over existing peer grading systems and discuss similarities and differences between those and MTA2 in section~\ref{sec:relatedwork}. Then, in section~\ref{sec:features}, we introduce the main features of MTA2 and how they work. We explain the user-interface and basic functionality of MTA2 in section~\ref{sec:userinterface}. %In Section~\ref{sec:backend}, we briefly go over the code base of MTA2, its general structure, and explain the way some of its core algorithms can be modified.  
Finally, we conclude this paper in Section~\ref{sec:conclusion}, where some future directions are also discussed. 



\begin{table*} [ht]
\centering
 \begin{tabular}{||c c c c c c c c||} 
 \hline
 - & PeerScholar & PG & CPR & CrowdGrader & PeerGrade & MTA1 & MTA2 \\  
 \hline\hline
 Incentivizing accurate grading by TA Spot checks & - & - & - & - & - & \checkmark & \checkmark \\
 \hline
 Standardization via calibration submissions & -  & - & \checkmark &- & - & \checkmark & \checkmark \\
 \hline
 Leverage reliable graders by having multiple pools & - & - & - & - & - & \checkmark & \checkmark \\
 \hline
 Allowing instro, auctors to choose the features there other topics you should also list? (E.g.,y want  & \checkmark  & - & \checkmark & \checkmark & \checkmark & - & \checkmark \\ 
 \hline
 Allowing instructors to chan students appeal? Can students see their grades? What about thege system logic  & - & - & - & - & - & - & \checkmark \\ 
 \hline
 The support for different assignment types & -  & \checkmark & - &\checkmark & \checkmark & - & \checkmark \\
 \hline
 The support four new features described at the beginning of the introduction?)flagging individual reviews & - & - & - & - & \checkmark & - & \checkmark \\
 \hline
\end{tabular}
\caption{Comparison between different peer grading applications}
\label{table:comparison}
\end{table*}

==> MTA2 paper- Arxiv/userinterface.tex <==

%This section describes the different parts of the MTA2 user interface, and thus the system workflow. %Most of the features presented in this section are the core of any peer grading system and are shared between most of them. %The goal here is to present the way such a feature is implemented in MTA2. 
%
When a user logs into MTA2, they see a list of the courses they are associated with and the role they have in each. Users can associate themselves with a new course by entering a given code.
%~(see Figure~\ref{fig:enrol}).
Upon choosing a course, every user sees an interface divided into four main tabs: dashboard, assignment, review, and appeal. %In the remainder of this section, we explain these tabs for different users. 
%\begin{figure*}[ht]
%    \centering
%    \includegraphics[scale=0.3]{images/enrol.png}
%    \caption{Course list and enrollment}
%    \label{fig:enrol}
%\end{figure*}

\subsection{Dashboard}
The dashboard is a one-screen overview shown at login; for instructors, it shows assigned tasks, a summary of course statistics, and a link to a list of all students~(see Figure~\ref{fig:dashboard_tab} on the left). By clicking on a student's name in this list, TAs and instructors can see every task that the chosen student has done throughout the course and the corresponding grades they were given. Finally, the course configuration (course name, visibility to students, enrollment codes, etc) can be viewed; which can only be edited by the instructors.

For students, the dashboard contains two main tables, as illustrated in Figure~\ref{fig:dashboard_tab} on the right. The first  shows  assigned tasks and deadlines. The second shows grades for previous assignments. Students can view their submissions and their reviews in detail by clicking on the associated grade. They can also appeal or flag a review if necessary. Student reviews are only available after the student review deadline is passed. The final score of each submission is shown once the TA review deadline is reached. (Observe that TAs might spot check an assignment and thereby change the assigned grade.) When multiple pools are enabled, the dashboard also indicates whether the student is supervised or independent.  


    % \begin{figure*}[t]
    %     \centering
    %     \includegraphics[scale=0.25 ]{images/student_dashboard_2.png}
    %     \caption{The student dashboard.}
    %     \label{fig:student_dashboard}
    % \end{figure*}
    

%\begin{figure}
%    \centering
%    \includegraphics[scale=0.3]{images/editconfiguration.png}
%    \caption{Edit course configuration}
%    \label{fig:editconfig}
%\end{figure}
\subsection{The Assignment tab}

Instructors and TAs can see the list of all assignments and create new ones using this tab. They can also view the submissions for each assignment by displaying the submission list. Instructors can furthermore determine whether an assignment is visible to students and set deadlines. 

For students, the Assignment tab shows students the list of their assignments; for assignments that are not yet due, students can edit their submissions. Students can also see and appeal their grades in this tab once the deadline for TA reviews has passed. 

\subsection{The Reviews tab}

Reviewing an assignment means reading a submitted piece of work and then completing a rubric. 
Rubric questions ask graders to evaluate an assignment in a particular dimension by choosing the most appropriate among a set of multiple choices. Each rubric question can also have a reasoning field, which asks the grader to provide a rationale for their choice. The rationale field can be set to require entries between a minimum and maximum length.

Submitted reviews can later be evaluated by TAs (using a different rubric). Instructors and TAs can assign reviews and evaluations, create rubrics, and see review stats from the review tab.
%~(see Figure~\ref{fig:review_tab_ta}). %The way the reviews can be assigned in MTA2 are illustrated in Figures~\ref{fig:assign_review} and \ref{fig:assign_ta_review}. 
If an assignment has more than one question, it is possible to assign different TAs to grade different questions. The algorithm used to assign TAs to assignments or to assign spot checks can be changed straightforwardly.
%\begin{figure*}[ht]
%    \centering
%    \includegraphics[scale=0.27]{images/review_tab_ta.png}
%    \caption{Review tab for Instructors/TAs}
%    \label{fig:review_tab_ta}
%\end{figure*}
%\begin{figure*}[ht]
%    \centering
%    \includegraphics[scale=0.32]{images/assign_review.png}
%    \caption{Assign student reviews in MTA2}
%    \label{fig:assign_review}
%\end{figure*}
%\begin{figure*}[ht]
%    \centering
%    \includegraphics[scale=0.32]{images/assign_ta_review.png}
%    \caption{Assign TA reviews in MTA2}
%    \label{fig:assign_ta_review}
%\end{figure*}

Instructors and TAs can also access the list of submitted reviews and view each one from this tab. %Figure~\ref{fig:review_example} shows an example of a review displayed in MTA2. 
When viewing a student review, instructors and TAs can request an evaluation for the review. Note that review evaluation is most naturally part of the spot-checking process. However, if instructors or TAs encounter a review that requires evaluation (e.g., via an appeal), they can also do so directly.



For students, the reviews tab displays two tables: one that shows pending reviews that the student still needs to submit and another that shows reviews that the student has previously submitted. The students can still edit their submitted reviews until the review deadline.
%~(see Figure~\ref{fig:rubric_question}).  
%\begin{figure*}[ht]
%    \centering
%    \includegraphics[scale=0.25]{images/rubric_question.png}
%    \caption{Rubric question creation}
%    \label{fig:rubric_question}
%\end{figure*}

\subsection{The Appeals tab}
\label{subsec:appeals}
%\begin{itemize}
%    \item what is the goal of appeal?
%    \item how it is done in MTA2?
The appeals tab shows each TA the appeals that are assigned to him or her along with their current status. They can also reassign an appeal that they cannot resolve themselves. Instructors can see all the appeals. For students, the appeals tab keeps track of all previously submitted appeals and their current status. New appeals are submitted via the assignment tab.
%    \begin{figure*}[ht]
%        \centering
%        \includegraphics[scale=0.2]{images/appeals.png}
%        \caption{Appealing interface in MTA2}
%        \label{fig:appeal}
%    \end{figure*}
%    \item what are some future directions?
%\end{itemize}

\subsection{Admin interface}
Certain instructors or TAs can be designated as administrators, meaning that they are afforded fine-grained control over course data via \href{https://docs.djangoproject.com/en/dev/ref/contrib/admin/}{Django Admin} interface, which is accessed via a fifth tab, ``Administration''. This interface allows for searching and filtering the data, and can be customized with new filters. It can also be used for data entry and manipulation. While this feature is not designed to be used frequently in production, it can be useful for testing or trying out new ideas. 




==> test.tex <==


%    \item What Peer grading is, how it helps, what the challenges are.

%\farzad{Apparently, the use of slash ("/") is not recommended in formal writing.} 


Peer grading can help students learn course material better by thinking critically about the work of their classmates. It can also make class sizes scalable by reducing a large portion of grading work for teaching assistants (TAs) and instructors~\citep{sadler2006impact}. However, there are many issues that can stop a peer grading system from achieving these desirable properties in practice, e.g., it is not clear how to make sure that students take their grading tasks seriously or that they know how to grade fairly. 






Many implementations of peer grading systems already exist~\citep{de2014crowdgrader,Calibratedpeerreview,wright2015mechanical,Peergrade}, which either work under the assumption that there is no access to teaching TAs at all or use TAs at a very basic level (e.g., resolving student appeals). However, for the reasons that will be explained in this paper, none of these systems can satisfy all the properties that a reliable peer grading system should have to be confidently used in practice.


\emph{Mechanical TA 2} (MTA2) is a peer grading application designed and developed to overcome practical issues associated with peer grading by leveraging limited access to teaching assistants (TAs). The first implementation of MTA (MTA1),  which was used in a computer science course called ``Computers and Society'' for several years significantly reduced the need for TA labor in a large class, and helped students grade more accurately and better learn the course material ~\citep{wright2015mechanical}. However, the design of the first version was specific to the course it was being used for and was not easy to revise or change, which made it difficult to try in other settings. MTA2 is created based upon MTA1 to resolve its limitations and also to be a reliable and flexible peer grading application which can be used in various different settings. %It is easy to modify for courses with different requirements and supports new features that are helpful to have in a practical peer grading system. 
%In many scenarios such as university classes, the instructor indeed has access to a limited TA resource. 

%Similar to MTA1, TAs play a limited but important role in obtaining reliable grades in MTA2. 



In many peer grading systems, students can appeal unfair grades so that no reviewer can get away with giving grades that are too low~\citep{de2014crowdgrader,Peergrade}. Furthermore, to better incentivize accurate grading, some systems reward their students based on a similarity measurement between grades given by them and by those given by their peers to same submissions~\citep{de2014crowdgrader,hamer2005method}. Unfortunately, collusion between students can trick both of these mechanisms: students can give unfair, but close to full mark grades to every single submission~\citep{de2016incentives,gao2016incentivizing}. This, in turn, dis-incentivizes students from spending time on their grading duties. Experimental studies have shown that this indeed happens in practice~\citep{gao2014trick}. 
\farzad{We can mention that even in the absence of collusion, grading students by closeness of their grade to their peers leads to a "race to mediocrity" (Keynesian Beauty contest).}
\hedayat{Sure, go ahead and do so. Then, we can decide if we want to keep it} MTA2 uses the idea of \emph{spot checking} to detect and avoid defective grading behavior such as collusion. Spot checking is the process of randomly choosing a fraction of submissions and having them graded by TAs. Once a submission is spot checked, a TA grades the submission carefully, evaluates the reviews given to that submission, and rewards or punishes the students based on how close their grades are to the TA assigned grade. If the system spot checks enough submissions, bad grading behaviors such as collusion are likely to be caught, therefore, instead of cheating, students would prefer to focus on their grading duties~\citep{de2016incentives,gao2016incentivizing}. 

%To obtain accurate grading and avoid students' collusion, MTA2 takes advantage of the limited availability of TAs in three main ways: 

A reliable peer grading system should also educate students on how to grade consistently and accurately. Without such an education, it is very likely that because of having different expectations, students would assign different grades to the same work~\citep{wright2015mechanical,wang2019your,Calibratedpeerreview}. MTA2 resolves this issue by two different TA-based approaches. The first approach is to ask students to review \emph{calibration} submissions, which are TA graded submissions from previous years. Once a student finishes grading a calibration submission, they immediately see the TA grade and how different they are from it and can calibrate their grading, accordingly. Such immediate feedback is an efficient way to improve one's performance~\citep{kulik1988timing}. The second approach is to let TAs evaluate reviews given by students to their peers at any time, if necessary (e.g., during an appeal or spot check process). %\farzad{I never understood how this happens. TAs are busy, I imagine they would look at an assignment only if there was an appeal/flag.} 
Although providing such feedback inevitably takes longer in this approach, TAs can look at a review given by a student to a submission and give direct feedback on how the submitted review could be improved.   

Even after performing calibration reviews and getting feedback from TAs, not every student is going to qualify for grading their peers accurately. At the same time, an efficient peer grading system should take advantage of those students whose grading performances reach a certain level of proficiency; Once a few of qualified students grade a submission, it is very likely that there is no more need for a TA to look at the submission. MTA2 takes this scenario into consideration by allowing instructors to divide students into two pools: independent and supervised, where students in each pool are only assigned to grade those in the same pool. Every submission and review submitted by students in the supervised pool will also be graded by a TA. At this stage, students are learning to be fair and consistent graders. At the beginning of the course, all students are in a supervised pool. However, supervised students have the ability to move to the independent pool by showing consistent performance either by accurately grading a set of calibration submissions or by being evaluated by TAs multiple times. After a student gets into the independent pool, their grading will be evaluated by TAs only if they are spot checked, the submission they have graded is appealed, or their review is flagged as inappropriate. 

%Spot checking also results in a fraction of final grades be TA grades in the system, which are expected to be more accurate than peer grades. Therefore, overall, the system would end up having more accurate grades.  

MTA2 improves MTA1's performance and usability by introducing new features. One of the key new features of MTA2 is its modular design. As mentioned, MTA1 used several helpful features such as spot-checking to build a more reliable peer grading system. Such features are helpful to have in a peer grading system, however, not every instructor can afford to have them in their course. The modularity of MTA2 lets instructors choose the features they want based on the workload of their courses. Another important usage for MTA2's modular design is that it makes MTA2 a good environment for testing different peer grading mechanisms. There are many important unanswered questions about building a practical peer grading system. For example, as mentioned, MTA's way of incentivizing accurate grading among students is to spot check them. However, finding the most efficient spot checking mechanism is still an open problem in many scenarios~\citep{zarkoob2019report}. MTA2 has not only made it easier for instructors to choose the features they want, but also to modify and test them in practice. To our knowledge, MTA2 is the first peer grading aplpication with such flexibility. %For example, an instructor can change the way that submissions are distributed among peers for grading or modify the algorithm by which spot checks are assigned, without having to worry about the functionality of other parts of the system.
 
 
In peer grading, grade aggregation methods can be such that having only one unfair grade would not affect students' final grade by much~\citep{hamer2005method}, e.g. by taking the median of reported grades from multiple students. This means that students are not motivated to appeal when they have only one unfair review. However, this should not mean that individual inappropriate reviews would remain hidden from the system. In our early experiments with MTA2, we observed that indeed this scenario happens frequently in practice. Therefore, we added a feature which lets students flag individual inappropriate reviews. % When a grade is appealed, a TA looks at the reasoning and if necessary and regrades the student's submission. The TA can also evaluate any of the reviews done for this submission. But, flagging individual inappropriate reviews is
This gives an opportunity for students to let the system know about inappropriate reviews without going through the whole appealing process. %\farzad{Can't we just do this computationally? I thought flagging was mostly used for "inappropriate" reviews (rude, etc?).}

 

%MTA2's flexibility along with some additional features help the system to work better in practice and also serve as a testbed for experimenting with different peer grading mechanisms.
%and was done in a way that the logic and the user-interface of the system were mixed together.  
%Although 

 
In addition to the modular design and the ability to flag individual reviews, MTA2 supports several other new features that extend its usability in various courses. First, while in MTA1 students could only input their solutions in a text-box, MTA2 supports various assignment formats, i.e., text, PDF, and quiz (multiple choice questions). Depending on the assignment type, MTA2 allows students to input text, upload a file, or choose one of the multiple choices as their solution. In the case of uploading text, PDF, or code files, uploaded files are rendered and shown directly in the browser without needing to be downloaded. Second, MTA2 allows instructors to upload a group of students submissions as a single zip file. This feature would be helpful for exams and quizzes outside the MTA2 framework, allowing them to be peer-graded as well. %All an instructor has to do to make this happen is to create an assignment in MTA2 and upload PDFs of scanned student submissions \farzad{too much detail, I suggest cutting off "named by students' usernames "} as a single zip file. 
Finally, MTA2 has a more advanced CAS and SAML2 integration, which allows users to login using their organizational accounts (e.g., university-wide login systems), without the need for creation of separate username and passwords.
 
     
   
The remainder of this paper is as follows. First, we go over existing peer grading systems and discuss similarities and differences between those and MTA2 in section~\ref{sec:relatedwork}. Then, in section~\ref{sec:features}, we introduce the main features of MTA2 and how they work. We explain the user-interface and basic functionality of MTA2 in section~\ref{sec:userinterface}. %In Section~\ref{sec:backend}, we briefly go over the code base of MTA2, its general structure, and explain the way some of its core algorithms can be modified.  
Finally, we conclude this paper in Section~\ref{sec:conclusion}, where some future directions are also discussed. 



\begin{table*} [ht]
\centering
 \begin{tabular}{||c c c c c c c c||} 
 \hline
 - & PeerScholar & PG & CPR & CrowdGrader & PeerGrade & MTA1 & MTA2 \\  
 \hline\hline
 Incentivizing accurate grading by TA Spot checks & - & - & - & - & - & \checkmark & \checkmark \\
 \hline
 Standardization via calibration submissions & -  & - & \checkmark &- & - & \checkmark & \checkmark \\
 \hline
 Leverage reliable graders by having multiple pools & - & - & - & - & - & \checkmark & \checkmark \\
 \hline
 Allowing instro, auctors to choose the features there other topics you should also list? (E.g.,y want  & \checkmark  & - & \checkmark & \checkmark & \checkmark & - & \checkmark \\ 
 \hline
 Allowing instructors to chan students appeal? Can students see their grades? What about thege system logic  & - & - & - & - & - & - & \checkmark \\ 
 \hline
 The support for different assignment types & -  & \checkmark & - &\checkmark & \checkmark & - & \checkmark \\
 \hline
 The support four new features described at the beginning of the introduction?)flagging individual reviews & - & - & - & - & \checkmark & - & \checkmark \\
 \hline
\end{tabular}
\caption{Comparison between different peer grading applications}
\label{table:comparison}
\end{table*}
